Efficient Conversational Search via Topical Locality in Dense Retrieval

Pre-trained language models have been widely exploited to learn dense representations of documents and queries for information retrieval. While previous efforts have primarily focused on improving effectiveness and user satisfaction, response time remains a critical bottleneck of conversational search systems. To address this, we exploit the topical locality inherent in conversational queries, i.e., the tendency of queries within a conversation to focus on related topics. By leveraging query embedding similarities, we dynamically restrict the search space to semantically relevant document clusters, reducing computational complexity without compromising retrieval quality. We evaluate our approach on the TREC CAsT 2019 and 2020 datasets using multiple embedding models and vector indexes, achieving improvements in processing speed of up to 10.4X with little loss in performance (4.4X without any loss). Our results show that the proposed system effectively handles complex, multiturn queries with high precision and efficiency, offering a practical solution for real-time conversational search.

==> makefile <==
### Makefile for LaTeX under Mac OS X
### Author: Franco Maria Nardini (francomaria.nardini@isti.cnr.it)
# pdflatex, textmate, and skim are needed to run properly all the commands here.

# Some assumptions:
# ./img: is the directory containing images
# ./style: is the directory containing the .cls and .sty

# NAME OF THE MAIN FILE (WITHOUT .tex)
BASEFILENAME=paper

# NAME OF THE BIBLIO FILE (WITHOUT .bib)
BIBLIOFILENAME=biblio

# NAME OF THE CAMERA READY FILE (WITHOUT .pdf)
DESTFILENAME=

# NAME OF THE COVER LETTER FILE (WITHOUT .pdf)
COVERFILENAME=


${BASEFILENAME}.pdf: *.tex ${BASEFILENAME}.aux ${BASEFILENAME}.bbl
	@pdflatex ${BASEFILENAME}.tex
	@open -F -a skim ${BASEFILENAME}.pdf &

${BASEFILENAME}.aux: *.tex
	@pdflatex ${BASEFILENAME}.tex

${BASEFILENAME}.bbl: ${BIBLIOFILENAME}.bib
	@bibtex ${BASEFILENAME}
	@pdflatex ${BASEFILENAME}.tex

all:
	@make clean
	@make pdf
	@make open

pdf:
	@pdflatex ${BASEFILENAME}.tex
	@bibtex ${BASEFILENAME}
	@pdflatex ${BASEFILENAME}.tex
	@pdflatex ${BASEFILENAME}.tex

open:
	@open -F -a skim ${BASEFILENAME}.pdf

pdf-cameraready:
	@pdflatex ${BASEFILENAME}.tex
	@pdflatex ${BASEFILENAME}.tex
	@mv ${BASEFILENAME}.pdf ${DESTFILENAME}.pdf
	@open -F -a skim ${DESTFILENAME}.pdf

pdf-coverletter:
	@pdflatex ${COVERFILENAME}.tex
	@bibtex ${BASEFILENAME}
	@pdflatex ${COVERFILENAME}.tex
	@pdflatex ${COVERFILENAME}.tex
	@rm ${COVERFILENAME}.aux
	@rm ${COVERFILENAME}.log
	@open -F -a skim ${COVERFILENAME}.pdf

images:
	@for filename in `ls ./img/*.eps`; do epstopdf $$filename; done;

count:
	@pdftotext ${BASEFILENAME}.pdf WORDS
	@wc --words WORDS
	@rm -f WORDS

clean:
	@rm -f ./img/*~ *~ *spl .*.lb *loa *aux *dvi *maf *mtc *mtc0 *log *fls *lof *lot *out *pdf *bbl *blg *ps *idx *toc *fdb_latexmk *synctex.gz *auxlock *cut

chkrefs:
	@bibtex ${BASEFILENAME}

tgz:
	@tar -czf $(PWD)\ `date +%Y%m%d%H%M`.tar.gz *tex *tmproj *bib ./img/* ./style/*

svn-commit:
	@svn update
	@svn commit -m "`date +%Y%m%d%H%M` - FM"

svn-update:
	@svn update

git-commit-push:
	@git commit -am "`date +%Y%m%d%H%M` - FM"
	@git push origin master

git-pull:
	@git pull origin master



==> sections/02-related.tex <==
% !TEX root = ../paper.tex
% !TeX spellcheck = en_US

\section{Related Work}
\label{sec:related}

An initial theoretical framework for conversational information retrieval was proposed by Radlinski \& Craswell \cite{10.1145/3020165.3020183}. Consequently, various aspects of this emerging field have been explored such as context tracking and query rewriting, previously done by custom models and generating explicit reformulations \cite{elgohary-etal-2019-unpack, 10.1145/3397271.3401130, MELE2021102682, 10.1145/3397271.3401268}, and later, through prompting now highly effective LLMs \cite{10350178, 10839752}. Knowledge-based conversational search systems have been explored, highlighting the need for complex question answering and conversational browsing capabilities \cite{vakulenko2019knowledgebasedconversationalsearch}. To balance search quality and efficiency, a reward-free conversation policy imitation learning framework has been developed, along with a new evaluation metric called Expected Conversational Reciprocal Rank (ECRR) \cite{wang2023rewardfreepolicyimitationlearning}. 

Thanks to the great representational capabilities of dense models, a step forward towards dense conversational search has been made. While rather costly in terms of efficiency, their capacity to incorporate context and embed entire conversations has driven this research field to achieve comparable results to LLMs query rewriting and state-of-the-art models.

One of the first models to be introduced is ConvDR \cite{10.1145/3404835.3462856}, a few-shot approach using a teacher-student framework to learn contextualized embeddings for multi-turn queries. Building on this, HAConvDR \cite{mo2024history} proposed context-denoised query reformulation and automatic mining of supervision signals to enhance history modeling, particularly for long conversations. To address data scarcity, ConvTrans \cite{mao-etal-2022-convtrans} developed a method to transform web search sessions into conversational search sessions, reducing reliance on manually generated data. Similarly, CONVERSER \cite{huang-etal-2023-converser} leveraged large language models to generate synthetic conversational queries from passages, achieving comparable performance to fully-supervised models with only a few in-domain examples. In CQE \cite{lin-etal-2021-contextualized} authors integrate conversational query reformulation directly into a dense retrieval model, optimizing a learning-to-rank loss over a dataset composed of weak labels. These approaches collectively aim to improve the effectiveness of conversational dense retrieval by addressing challenges in data availability, context understanding, and query reformulation. Custom conversational sparse models are also proposed, such as CoSPLADE \cite{10.1007/978-3-031-28244-7_34}. It uses a CANARD-tuned lightweight first-stage ranked based on SPLADE and a stage ranked based on MONO T5.

In recent years, the application of Large Language Models (LLMs) in the realm of conversational search 
%has garnered significant attention due to their ability to interpret and respond to complex user queries effectively. LLMs demonstrate strong generalization capabilities, making them well-suited for dense retrieval tasks in multi-turn conversational contexts. 
includes contrastive learning techniques and session-based tuning methods.
These advancements have shown promising results in improving the accuracy and robustness of conversational search systems, outperforming traditional retrieval models. The development of systems like ChatRetriever \cite{mao-etal-2024-chatretriever} highlights the potential of LLMs to revolutionize conversational search by providing more accurate, context-aware responses, thereby advancing the field and opening new avenues for further research.
%Understanding user intent in multi-turn conversational searches is crucial. 
The model employs a dual-learning approach, using contrastive learning for retrieval and masked instruction tuning for better session understanding. 
%The work highlights the potential of adapting LLMs for complex input retrieval and offers an effective method for advancing this field.
% Experiments on five benchmarks show that ChatRetriever surpasses existing models, matching the performance of LLM-based rewriting methods and demonstrating robustness in diverse conversational contexts. 

%Conversational search requires accurate interpretation of user intent from complex multi-turn contexts. This paper presents ChatRetriever, which inherits the strong generalization capability of large language models to robustly represent complex conversational sessions for dense retrieval. To achieve this, we propose a simple and effective dual-learning approach that adapts LLM for retrieval via contrastive learning while enhancing the complex session understanding through masked instruction tuning on high-quality conversational instruction tuning data. Extensive experiments on five conversational search benchmarks demonstrate that ChatRetriever substantially outperforms existing conversational dense retrievers, achieving state-of-the-art performance on par with LLM-based rewriting approaches. Furthermore, ChatRetriever exhibits superior robustness in handling diverse conversational contexts. Our work highlights the potential of adapting LLMs for retrieval with complex inputs like conversational search sessions and proposes an effective approach to advance this research direction.

Contrasting approaches that primarily leverage human-rewritten queries as labels to train query rewriting models, Ye et al. \cite{ye-etal-2023-enhancing} propose utilizing large language models (LLMs) as query rewrites after having proposed four essential properties for well-formed rewrites. They also propose distilling the rewriting capabilities of LLMs into smaller models to reduce rewriting latency. The prompting framework LLM4CS \cite{mao-etal-2023-large} leverages LLMs as a text-based search intent interpreter to help conversational search. Recently, large language models (LLMs) have demonstrated amazing capabilities for text generation and conversation understanding. The performance evaluation includes an extensive automatic and human evaluation on three conversational search benchmarks, CAsT-19, CAsT-20, and CAsT-21, and demonstrates the effectiveness of the approach. In \cite{10350178}, authors also provide a few-shot LLM prompting approach that achieves exceeding performance over other state-of-the-art models and that of human-rewritten queries.

While the use of LLMs either for promoting or for creating dense representations has driven the field of conversational search to impressive results, it is without a doubt that resource concerns have been raised. Although highly effective in resolving context tracking and user intent, the resources required for creating the query rewritings (either sparse or dense) have been mentioned in papers such as \cite{lin-etal-2021-contextualized}. 

On the other hand, there is very little work regarding efficiency during the search process. In \cite{10.1145/3578519} authors propose a model for a client-server architecture for optimizing requests by introducing a client-side cache. Results show the method is effective, and conversational search presents some characteristics that can expedite response time in specific conditions.

Capitalizing on those observations, this work proposes a framework for efficient conversational dense retrieval that exploits the semantic relatedness of queries in a conversation to limit the search to specific parts of the index, supposedly closer to the conversation, in the embedding space.


==> sections/11-framedEnvs.tex <==
\noindent \textbf{Framed Environments}

\fquestion{domanda}

\fnote{nota}

\ftodo{nota}

\freply{risposta}

\noindent \textbf{Inline Environments}

\iquestion{nota}

\inote{nota}

\ireply{nota}

\itodo{nota}

\missingcite{}

\missingref{}

\noindent \textbf{Revision Commands}

\fm{nota}
\fmchange{nota}{nota2}


